SiFall: Practical Online Fall Detection with RF Sensing

Falls present a significant global public health challenge, especially in today's aging society, underscoring the importance of developing an effective fall detection system. Non-invasive radio-frequency (RF) based fall detection has garnered substantial attention due to its wide coverage and privacy-preserving nature. Existing RF-based fall detection systems approach falls as an activity classification problem, assuming that human falls introduce reproducible patterns to the RF signals. However, we argue that falls are inherently accidental, making their impact uncontrollable and unforeseeable. We propose a fundamentally different approach to fall detection by shifting the focus from directly identifying hard-to-quantify falls to recognizing normal, repeatable human activities, thus treating falls as abnormal activities outside the normal activity distribution. We introduce a self-supervised incremental learning system incorporating FallNet, a deep neural network that employs unsupervised learning techniques. Our real-time fall detection system prototype leverages WiFi Channel State Information (CSI) sensing data and has been extensively tested with 16 human subjects.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

==> seg.tex <==
\subsubsection{Fall-like Activities Segmentation}
Falls changes the status of the human body within a short time, causing sudden and sharp signal variation.
As a result, the 

and thus introduces high frequency components to the signal variations.
Although $d(t)$ is robust to detect human motions, fall detection requires a more fine-grained analysis, such as examining the instantaneous velocity of a motion. A common practice to detect fall is to apply time-frequency analysis (e.g., Short-time Fourier Transform (STFT)) to $d(t)$ by using the signal frequency under a small time window $w$ to approximate the instantaneous velocity. However, the computational overhead of constantly performing STFT on $d(t)$ is unaffordable due to SiFall's real-time requirement. 
%and even the presence of high-frequency components is still not sufficient to directly identify falls. 
%\subsection{Reverse Segmentation Strategy}
%The amount of paths variation 
%between falls and fall-like movements, further refinement is needed. SiFall proposes a backtracking dynamic segmentation algorithm based on a coarse-to-fine strategy that works in a light-weight manner to meet the real-time requirements.
%A typical way to distinguish falls is to obtain features that represent human instant velocity. 
%Time-frequency analysis, such as Short-time Fourier Transform, STFT, that is widely adopted as a typical way to identify high frequency component as the core feature of falls.
%Furthermore, the parameter selection of the two window size, a motion signal length $W$ and the time resolution $w$, is vital to STFT result and prevent SiFall from utilizing dynamic signal segments.
Therefore, SiFall proposes a lightweight indicator $\vec{v}$ to capture high-frequency component vicariously. $\vec{v}$, a second-order derivative approximation of $d(t)$, is obtained by computing the moving variance twice in a small sliding window of sample length $k$, which quantifies the instant channel variation of its dynamic component. Thus, $\vec{v}$ is able to identify potential fall activities.

% $vec{v}$ is calculated twice by finding the standard deviation in a small sliding window  and finding the standard deviation again for its result to approximate the second order derivative 
% $d(t)$
\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth,scale = 0.98]{Figures/fig3.PNG}
  \caption{An example trace of $d(t)$ and its corresponding $\vec{v}$ and the time-frequency spectrum.}
  \vspace{-0.3cm}
  \label{fig:item}
\end{figure}

Figure~\ref{fig:item} shows an example trace of $d(t)$ together with its STFT spectrum result and the corresponding $\vec{v}$ values. %Here, WT is chosen over STFT because WT uses a mother wavelet function that can be scaled and shifted, thus having a finer and more comprehensive visual presentation.
%short windows $w$ at high frequencies and long windows $w$ at low frequencies to obtain fine-grained time-frequency information for visualization whereas STFT has the drawback of requiring fixed window size.
%, which may introduce bias when we decide the window size.
Comparing $\vec{v}$ and STFT spectrum in Figure~\ref{fig:item}, the high frequency component occurs in the spectrum is analogous with the large value occurs in $\vec{v}$ despite the absence of fine-grained information in $\vec{v}$. Therefore, $\vec{v}$ is sufficient to identify intensity motions with the benefit of low computational overhead.
The computing time of $\vec{v}$ is $45\times$ faster than STFT\footnote{This is the result of averaging over 10,000 packets at a sampling rate of 20Hz. The execution time calculated by Matlab tic-toc function.}. STFT known as the relatively faster time-frequency analysis method compared with WT and other typical methods~\cite{yan2020comparison}. 
As a large $\vec{v}$ value indicates intensity motions, i.e. potential falls, the corresponding $d{(t)}$ of the activities are segmented out by the dynamic backtracking segmentation algorithm then performing STFT on it to obtain the detailed time-frequency information.
%in fact helps to scan potential falls, allowing the time-frequency analysis to target only potential falls and thus save computation significantly.

%怎么 perform
In particular, $\vec{v}$ is used to help to identify the start and end time points of fall-like activities and thus obtaining a sequence of $d(t)$ that is the channel variations caused by human motion in the corresponding time period.
%the backtracking dynamic segmentation algorithm to cut over the associated signal $d(t)$ then time-frequency analysis is only be performed over the segmented signal $d(t)$. 
Although the start of an activity is difficult to detect on the sequence of signal samples, fall-like activities usually end with a temporary stationary state, which provides a reference time point for backtracking the signal segment.
When the variance of $d(t)$ is estimated below a threshold, suggesting a stationary state, SiFall records the time $t_{end}$, then searching the maximum value of $\vec{v}$ in the previous five seconds. If there is $\vec{v}_{max}>\Theta$, another threshold, which suggests a relative intensity motion, SiFall records the corresponding time as $t_{max}$. After that, SiFall extract $d(t)$ between $\left [ t_{max}-3s, t_{end}+1s \right ]$ then performing STFT on it to obtain the segment's time-frequency spectrum. SiFall adopts "more is better than less" strategy to extract the segment, so the added three second time before $t_{max}$ is used to include the fall-like activity as complete as possible. The added one second after $t_{end}$ assumes the state after the fall may also contain information that can be utilized to refine the result. 
Note that the length of segments and their corresponding spectrum is variable because the time between $t_{max}$ and $t_{end}$ depends on the duration of the activity and is variable. Following that, the spectrum of the fall-like activity will be supplied to the neural network in the back-end for confirmative fall detection. 
%After capturing the potential fall with large $\vec{v}$, $\vec{v}$ serves as an indicator to trigger a dynamic segmentation algorithm cutting over the corresponding signal $d(t)$.and segment counterparts of $d(t)$. 
%STFT is only be performed over the , and the result   SiFall applies a backtracking approach to identify the boundary of each fall-like activity and therefore extract the corresponding signal segment.
%So far, the $\vec{v}$ alone is still insufficient for detecting falls, because there are other daily activities that can cause high frequency path changes, such as jumping, squatting, etc. which are collectively termed as fall-like activities in our paper. $\vec{v}$ however serves as a light-weight indicator for fall-like activities and filters out activities that are far from falls so the problem space is narrowed down. Nevertheless, the activity extractor is needed for further fined-grained feature differentiation. Recall that daily activities are performed continuously and casually, the boundary between activities is not given and ambiguous in RF signal, how to identify the boundary and cut out variable-length of signal that represents a activity is challenging. In view of the fact that the activity extractor is only an intermediate result and not the final result, which can be refined afterwards, thus SiFall adopts a strategy call "more is better than less" with the computational overhead trade of to design the opportunistic backtracking dynamic segmentation algorithm. 

 %The extracted segment of $d(t)$ will later go through STFT to derive finer-grained time-frequency information, which is finally fed to 
\begin{algorithm}

\caption{Fall-like Segmentation Algorithm}
\label{alg:seg}
\SetKwProg{generate}{Function \emph{generate}}{}{end}
\KwIn{$d(t)$; Threshold: $\Theta,\Gamma$; Small window size: $k$; $fs$}
$\vec{v}_{t}$ = movstd(movstd($d(t)$,$k$),$k$)\;
movstd($d(t)$,$k$) 

= std($d(t)$-$\left \lfloor k/2 \right \rfloor$, ..., $d(t)$, ..., $d(t)$+$\left \lfloor k/2 \right \rfloor$)

\If{movstd(d(t),k) < $\Gamma$;}
{record $t$ as $t_{end}$ \;

    \If{$max(\vec{v}_{t},\vec{v}_{t-5fs})$ > $\Theta$}
    {record $t_{m a x }$;\\
    temp = $[d(t_{max}-3fs), d(t_{end}+fs)]$;\\
    seg = STFT(temp)}}
% \generate{Object pivot}{
%      \ForAll{child $c$ in pivot}{
%      \If{ $c$'s FieldContext is not set and $c$ is fusible}{
%           generate($c$)\;
%       }
%      }
%      build pivot's fieldContext $fc$\;
%      EmitClassName\;
%      EmitFields($fc$)\;
%      EmitMethods($fc$)\;
%}
\end{algorithm}

%% boxes -- remove
% Meanwhile, as we use the amount of dynamic component variation to detect human movements and it serves as a trigger to cut out the fall-like activities. One may think whether an object falling from a height be judged as a fall. Therefore, we let three boxes of different sizes\footnote{Box1 is 6.61x3.66x2.05 inches with 0.2kg (small), box2 is 23.8x14.1x24.4 inches with 3.6kg (large) and box3 is 11.0x9.5x4.0 inches with 1.5kg (medium).} drop from 2 meters height and investigate its $d(t)$ and $\vec{v}$. As Figure~\ref{fig:item} shown, no matter it is $d(t)$ or $\vec{v}$, the pattern of item drop is far from human movements. Firstly, $\vec{v}$ of three items are all below the threshold for the fall-like movements. In addition, the value of $d(t)$ before and after the item drop almost remains the same. This is because compared with objects, people are larger reflectors, which causes changes in the multipath profile. 

% The time durations of object drop is significantly shorter than that of human activities. Consequently, SiFall is robust to object drops.

%%%% old text

% Human fall usually happens changes the status of the human body within a short time, causing sudden and sharp variations in signal $d(t)$.
% We therefore leverages such sudden variations as the fingerprint for identifying the falls and other fall-like activities.

% %Although $d(t)$ is robust to detect human motions, fall detection requires a more fine-grained analysis, 
% %such as examining the instantaneous velocity of a motion. 
% A common practice to detect sudden signal variations is 
% to apply time-frequency analysis (e.g., Short-time Fourier Transform (STFT)) to $d(t)$ 
% and then use the signal frequency under a small time window $w$ to approximate the instantaneous velocity. 
% However, the computational overhead of constantly performing STFT on $d(t)$ is unaffordable 
% due to \systemnames{} real-time requirement. 
%and even the presence of high-frequency components is still not sufficient to directly identify falls. 
%\subsection{Reverse Segmentation Strategy}
%The amount of paths variation 
%between falls and fall-like movements, further refinement is needed. SiFall proposes a backtracking dynamic segmentation algorithm based on a coarse-to-fine strategy that works in a light-weight manner to meet the real-time requirements.
%A typical way to distinguish falls is to obtain features that represent human instant velocity. 
%Time-frequency analysis, such as Short-time Fourier Transform, STFT, that is widely adopted as a typical way to identify high frequency component as the core feature of falls.
%Furthermore, the parameter selection of the two window size, a motion signal length $W$ and the time resolution $w$, is vital to STFT result and prevent SiFall from utilizing dynamic signal segments.
%Therefore, SiFall proposes a lightweight indicator $\vec{v}$ to capture high-frequency component vicariously. $\vec{v}$, a second-order derivative approximation of $d(t)$, is obtained by computing the moving variance twice in a small sliding window of sample length $k$, which quantifies the instant channel variation of its dynamic component. Thus, $\vec{v}$ is able to identify potential fall activities.

% $vec{v}$ is calculated twice by finding the standard deviation in a small sliding window  and finding the standard deviation again for its result to approximate the second order derivative 
% $d(t)$


%Figure~\ref{fig:item} shows an example trace of $d(t)$ together with its STFT spectrum result and the corresponding $\vec{v}$ values. %Here, WT is chosen over STFT because WT uses a mother wavelet function that can be scaled and shifted, thus having a finer and more comprehensive visual presentation.
%short windows $w$ at high frequencies and long windows $w$ at low frequencies to obtain fine-grained time-frequency information for visualization whereas STFT has the drawback of requiring fixed window size.
%, which may introduce bias when we decide the window size.
% Comparing $\vec{v}$ and STFT spectrum in Figure~\ref{fig:item}, the high frequency component occurs in the spectrum is analogous 
% with the large value occurs in $\vec{v}$ despite the absence of fine-grained information in $\vec{v}$. 
% Therefore, $\vec{v}$ is sufficient to identify intensity motions with the benefit of low computational overhead.
% The computing time of $\vec{v}$ is $45\times$ faster than STFT\footnote{This is the result of averaging over 10,000 packets 
% at a sampling rate of 20Hz. The execution time calculated by Matlab tic-toc function.}. 
% STFT known as the relatively faster time-frequency analysis method compared with WT and other typical methods~\cite{yan2020comparison}. 
% As a large $\vec{v}$ value indicates intensity motions, i.e. potential falls, 
% the corresponding $d{(t)}$ of the activities are segmented out by the dynamic backtracking segmentation algorithm then performing STFT 
% on it to obtain the detailed time-frequency information.
%in fact helps to scan potential falls, allowing the time-frequency analysis to target only potential falls and thus save computation significantly.

%怎么 perform
%  $\vec{v}$ is used to help to identify the start and end time points of fall-like activities 
% and thus obtaining a sequence of $d(t)$ that is the channel variations caused by human motion in the corresponding time period.
% %the backtracking dynamic segmentation algorithm to cut over the associated signal $d(t)$ then time-frequency analysis is only be performed over the segmented signal $d(t)$. 
% Although the start of an activity is difficult to detect on the sequence of signal samples, 
% fall-like activities usually end with a temporary stationary state, 
% which provides a reference time point for backtracking the signal segment.
